Physics Reasoner: Knowledge-Augmented Reasoning for Solving Physics Problems with Large Language Models

Physics problems constitute a significant aspect of reasoning, necessitating complicated reasoning ability and abundant physics knowledge. However, existing large language models (LLMs) frequently fail due to a lack of knowledge or incorrect knowledge application. To mitigate these issues, we propose Physics Reasoner, a knowledge-augmented framework to solve physics problems with LLMs. Specifically, the proposed framework constructs a comprehensive formula set to provide explicit physics knowledge and utilizes checklists containing detailed instructions to guide effective knowledge application. Namely, given a physics problem, Physics Reasoner solves it through three stages: problem analysis, formula retrieval, and guided reasoning. During the process, checklists are employed to enhance LLMs' self-improvement in the analysis and reasoning stages. Empirically, Physics Reasoner mitigates the issues of insufficient knowledge and incorrect application, achieving state-of-the-art performance on SciBench with an average accuracy improvement of 5.8%.

==> tables/table_formulaset.tex <==
\begin{table}[t]
\small
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{lc}

\toprule
Subfield   & Fornuma Number \\
\midrule
Fundamental Physics  &  47\\
Celestial Mechanics  & 11\\
Electricity & 22  \\
Thermo  &  42 \\
All  &  122\\
\bottomrule
\end{tabular}
% }
\caption{Statistics of formula count across different subfields in our formula set}
\label{tab: formulaset}
\end{table}
